The Hughes model for pedestrian dynamics and congestion modelling

In this paper we present a numerical study of some variations of the Hughes model for pedestrian flow under different types of congestion effects. The general model consists of a coupled non-linear PDE system involving an eikonal equation and a first order conservation law, and it intends to approximate the flow of a large pedestrian group aiming to reach a target as fast as possible, while taking into account the congestion of the crowd. We propose an efficient semi-Lagrangian scheme (SL) to approximate the solution of the PDE system and we investigate the macroscopic effects of different penalization functions modelling the congestion phenomena.

==> macro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                 TEX MACRO FILE, F. BONNANS
%                       APRIL 27, 2003
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\dd{{\rm d}}
\newcommand{\ddt}{\frac{\rm d}{{\rm d} t} }
\newcommand{\dotex}[1]{{\frac{\displaystyle d #1}{\displaystyle dt}}}
\newcommand{\ideal}[1]{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMPHAZISE, ETC 
\newcommand{\new}[1]{{\em #1}}
\newcommand{\newd}[2]{{\em #1}\index{#2}}
\newcommand{\prob}[1]{{\em #1}\index{#1}}
\newcommand{\mrm}[1]{\text{\rm #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GRAPHES 
% \newcommand{\arc}[2]{(#1,#2)}
\def\arcset{{\mathcal A}}
\def\nodeset{{\mathcal N}}
\def\incid{{M}}
\newcommand{\edge}[2]{\{#1,#2\}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DIVERS S. Gaubert

\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\arcm}[2]{#1#2}

\newcommand{\transp}{^\top}
\newcommand{\wglobal}[1]{\typeout{warning: #1 global definition}#1}
\newcommand{\promis}{\typeout{warning: verifier que c est fait}}
\newcommand{\ext}{\operatorname{extr}}
\newcommand{\co}{\operatorname{co}}
\newcommand{\cob}{\operatorname{\overline{co}}}
\newcommand{\set}[2]{\{#1\mid\,#2\}}

\newenvironment{sgdelicat}{\small}{}
\newenvironment{sgremarque}{\begin{remark}}{\hfill $\bullet$\end{remark}}

\def\weight(#1,#2){c_{#1,#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DIVERS RO
\def\Kh{\hat{K}} 
\def\Eb{\bar{E}}
\def\Adj{{\rm Adj}}
\def\Adjc{{\rm Adjc}}
\def\deg{{\rm deg}}
\def\red{{\rm red}}
\def\ra{{\rm ra}}
\def\ovdeg{{\overline{\rm deg}}}
\def\degu{\underline{\rm deg}}
\def\Mh {{\hat M}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% Prog Dyn
\def\qbo {{\bf q}}
\def\ubo {{\bf u}}
\def\ybo {{\bf y}}
\def\uv {{\underline v}}

%%%%%%%%%%%%%%%%%%%%%% FRENCH %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%   FRANCAIS / ANGLAIS
%%% VERSION FRANCAISE
\newcommand{\fa}[2]{#2}
% TEXTE
\newcommand{\Alors}{Alors }
\newcommand{\alors}{alors }
\newcommand{\alorsv}{alors, }
\newcommand{\avec}{avec }
\newcommand{\dans}{dans }
\newcommand{\debdem}{{\noindent \bf D\'emonstration.}\quad}
\newcommand{\et}{et }
\newcommand{\ett}{et }
\newcommand{\est}{est }
\newcommand{\ilexiste}{il existe }
\newcommand{\mesurable}{mesurable}
\newcommand{\ou}{ou }
\newcommand{\pour}{pour }
\newcommand{\pourtout}{pour tout }
\newcommand{\pp}{p.p. }
\newcommand{\quand}{quand }
\newcommand{\Si}{Si }
\newcommand{\si}{si }
\newcommand{\sinon}{sinon }
\newcommand{\Soient}{Soient }
\newcommand{\Soit}{Soit }
\newcommand{\soit}{soit }
\newcommand{\sur}{sur }
\newcommand{\telque}{tel que }
\newcommand{\telleque}{telle que }
\newcommand{\thm}{th\'eor\`eme }
\newcommand{\un}{un }
% MATHS
\newcommand\meas{\mathop{\rm mes}}
%\newcommand\rank{\mathop{\rm rang}}
%
%%% VERSION ANGLAISE
 \if {
  \renewcommand{\fa}[2]{#1}
% TEXTE
  \renewcommand{\Alors}{Then }
  \renewcommand{\alors}{then }
  \renewcommand{\alorsv}{then, }
  \renewcommand{\avec}{with }
  \renewcommand{\dans}{in }
  \renewcommand{\debdem}{\noindent {\bf Proof.}\quad}
  \renewcommand{\et}{and }
  \renewcommand{\ett}{and }
  \renewcommand{\est}{is }
  \renewcommand{\ilexiste}{there exists }
  \renewcommand{\mesurable}{measurable}
  \renewcommand{\ou}{or }
  \renewcommand{\pour}{for }
  \renewcommand{\pourtout}{for all }
  \renewcommand{\pp}{a.e. }
  \renewcommand{\quand}{when }
  \renewcommand{\Si}{If }
  \renewcommand{\si}{if }
  \renewcommand{\sinon}{otherwise }
  \renewcommand{\Soient}{Let }
  \renewcommand{\Soit}{Let }
  \renewcommand{\soit}{let }
  \renewcommand{\sur}{on }
  \renewcommand{\telque}{such that }
  \renewcommand{\telleque}{such that }
  \renewcommand{\thm}{theorem }
  \renewcommand{\un}{a }
% MATHS
  \renewcommand\meas{\mathop{\rm meas}}  
  \renewcommand\rank{\mathop{\rm rank}}
 } \fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\if { 
\renewcommand{\chapterl}[1]{\chapter{\LARGE \bf {#1}}\vspace{-40mm}}
\renewcommand{\sectionl}[1]{\section{\LARGE \bf {#1}}}
\renewcommand{\subsectionl}[1]{\subsection{\LARGE \bf {#1}}}
\renewcommand{\subsubsectionl}[1]{\subsubsection{\Large \bf {#1}}}
\renewcommand{\paragraphl}[1]{\paragraph{\LARGE \bf {#1}}}
\renewcommand{\subparagraphl}[1]{\subparagraph{\LARGE \bf {#1}}}

\renewcommand{\captionl}[1]{\caption{\LARGE \bf {#1}}}

\renewcommand{\Largel}{\Large}}{{\caption}}
} \fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\findem{\hfill{$\blacksquare$}\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%% PROOFS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\debdem}{\begin{proof}} \def\findem{\end{proof}}

%%% \newenvironment{proof}{{\noindent \bf D\'emonstration.}\quad}{\hfill{$\blacksquare$}\medskip}
\newenvironment{proofdu}[1]{{\noindent \bf D\'emonstration #1.}\quad}{\hfill{$\blacksquare$}\medskip}

%%% \newcommand{\qed}{\findem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HAT %%%%%%%%%%%%%%%%%%%%%%%%
\def\ah{\hat{a}}
\def\bh{\hat{b}}
\def\ch{\hat{c}}
\def\dh{\hat{d}}
\def\eh{\hat{e}}
\def\fh{\hat{f}}
\def\gh{\hat{g}}
\def\hh{\hat{h}}
\def\ih{\hat{i}}
\def\jh{\hat{j}}
\def\kh{\hat{k}}
\def\lh{\hat{l}}
\def\mh{\hat{m}}
\def\nh{\hat{n}}
\def\oh{\hat{o}}
\def\ph{\hat{p}}
\def\qh{\hat{q}}
\def\rh{\hat{r}}
\def\sh{\hat{s}}
\def\th{\hat{t}}
\def\uh{\hat{u}}
\def\vh{\hat{v}}
\def\wh{\hat{w}}
\def\xh{\hat{x}}
\def\yh{\hat{y}}
\def\zh{\hat{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BAR %%%%%%%%%%%%%%%%%%%%%%%%
\def\ab{\bar{a}}
\def\bb{\bar{b}}
\def\cb{\bar{c}}
\def\db{\bar{d}}
\def\eb{\bar{e}}
\def\fb{\bar{f}}
\def\gb{\bar{g}}
\def\hb{\bar{h}}
\def\ib{\bar{i}}
\def\jb{\bar{j}}
\def\kb{\bar{k}}
\def\lb{\bar{l}}
\def\mb{\bar{m}}
\def\nb{\bar{n}}
\def\ob{\bar{o}}
\def\pb{\bar{p}}
\def\qb{\bar{q}}
\def\rb{\bar{r}}
\def\sb{\bar{s}}
\def\tb{\bar{t}}
\def\ub{\bar{u}}
\def\vb{\bar{v}}
\def\wb{\bar{w}}
\def\xb{\bar{x}}
\def\yb{\bar{y}}
\def\zb{\bar{z}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UPPERCASE BAR %%%%%%%%%%%%%%
\def\Ab{\bar{A}}
\def\Bb{\bar{B}}
\def\Cb{\bar{C}}
\def\Db{\bar{D}}
\def\Eb{\bar{E}}
\def\Fb{\bar{F}}
\def\Gb{\bar{G}}
\def\Hb{\bar{H}}
\def\Ib{\bar{I}}
\def\Jb{\bar{J}}
\def\Kb{\bar{K}}
\def\Lb{\bar{L}}
\def\Mb{\bar{M}}
\def\Nb{\bar{N}}
\def\Ob{\bar{O}}
\def\Pb{\bar{P}}
\def\Qb{\bar{Q}}
\def\Rb{\bar{R}}
\def\Sb{\bar{S}}
\def\Tb{\bar{T}}
\def\Ub{\bar{U}}
\def\Vb{\bar{V}}
\def\Wb{\bar{W}}
\def\Xb{\bar{X}}
\def\Yb{\bar{Y}}
\def\Zb{\bar{Z}}

\def\Cbar{\bar{C}}
\def\Tbar{\bar{T}}
\def\Zbar{\bar{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TILDE %%%%%%%%%%%%%%%%%%%%%%%%

\def\at{\tilde{a}}
\def\bt{\tilde{b}}
\def\ct{\tilde{c}}
\def\dt{\tilde{d}}
\def\et{\tilde{e}}
\def\ft{\tilde{f}}
\def\gt{\tilde{g}}
\def\hit{\tilde{h}}
\def\iit{\tilde{i}}
\def\jt{\tilde{j}}
\def\kt{\tilde{k}}
\def\lt{\tilde{l}}
\def\mt{\tilde{m}}
\def\nt{\tilde{n}}
\def\ot{\tilde{o}}
\def\pt{\tilde{p}}
\def\qt{\tilde{q}}
\def\rt{\tilde{r}}
\def\st{\tilde{s}}
\def\tt{\tilde{t}}
\def\ut{\tilde{u}}
\def\vt{\tilde{v}}
\def\wt{\tilde{w}}
\def\xt{\tilde{x}}
\def\yt{\tilde{y}}
\def\zt{\tilde{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UPPERCASE TILDE %%%%%%%%%%%%%%%%
\def\tA{\tilde{A}} 
\def\tL{\tilde{L}} 
\def\tS{\tilde{S}} 
\def\tV{\tilde{V}} 
\def\tW{\tilde{W}} 
\def\tX{\tilde{X}} 
\def\tY{\tilde{Y}} 
\def\tZ{\tilde{Z}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BOLDFACE %%%%%%%%%%%%%%%%%%%%%%%
\def\ubf { {\bf u}}  
\def\vbf { {\bf v}}  
\def\wbf { {\bf w}}  
\def\xbf { {\bf x}}  
\def\ybf { {\bf y}}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAL %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cala{{\cal A}}
\def\calb{{\cal B}}
\def\calc{{\cal C}}
\def\cald{{\cal D}}
\def\cale{{\cal E}}
\def\calf{{\cal F}}
\def\calg{{\cal G}}
\def\calh{{\cal H}}
\def\cali{{\cal I}}
\def\calj{{\cal J}}
\def\calk{{\cal K}}
\def\call{{\cal L}}
\def\calm{{\cal M}}
\def\caln{{\cal N}}
\def\calo{{\cal O}}
\def\calp{{\cal P}}
\def\calq{{\cal Q}}
\def\calr{{\cal R}}
\def\cals{{\cal S}}
\def\calt{{\cal T}}
\def\calu{{\cal U}}
\def\calv{{\cal V}}
\def\calw{{\cal W}}
\def\calx{{\cal X}}
\def\caly{{\cal Y}}
\def\calz{{\cal Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% OTHER CAL %%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cL{{\cal L}}
\def\cP{{\cal P}}

\def\cPt{\widetilde{\cal P}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATHCAL %%%%%%%%%%%%%%%%%%%%%%%%
\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\N{\mathcal{N}}
\def\P{\mathcal{P}}
\def\Q{\mathcal{Q}}
\def\R{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\T{\mathcal{T}}
\def\U{\mathcal{U}}
\def\V{\mathcal{V}}
\def\W{\mathcal{W}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}
\def\Z{\mathcal{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% AUTRES MATHCAL %%%%%%%%%%%%%%%%%%
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sV}{\mathcal{V}}
%%%%%%%%%%%%%%%%%%%%%%% SPECIAL   %%%%%%%%%%%%%%%%%%%%%%%%
% NOTATION HAMILTONIEN
\def\HH{\overline{\bf H}}
%%%%%%%%%%%%%%%%%%%%%%% UNDERLINE %%%%%%%%%%%%%%%%%%%%%%%%
\def\xu{\underline{x}}
%
\def\uV{\underline{V}}

%%%%%%%%%%%%%%%%%%%%%%% GREEKS %%%%%%%%%%%%%%%%%%%%%%%%
\def\eps{\varepsilon}
\def\Om{{\Omega}}
\def\om{{\omega}}
\def\ml{\lambda}
\def\mlb{\bar{\lambda}}
\def\mub{\bar{\mu}}
\def\nub{\bar{\nu}}
\def\taub{{\bar\tau}}
%%%%%%%%%%%%%%%%%%%%%%%% MATH OPERATORS %%%%%%%%%%%%%%%%
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\def\ad{\mathop{\rm ad}}
\def\affhull{\mathop{\rm affhull}}
\def\argmin{\mathop{\rm argmin}}
\def\argmax{\mathop{\rm argmax}}
\def\cl{\mathop{\rm cl}}
\def\cone{\mathop{\rm cone}}
\def\conv{\mathop{\rm conv}}
\def\convbar{\mathop{\rm \overline{conv}}}
\def\deg{\mathop{\rm deg}}
\def\det{\mathop{\rm det}}
\def\diag{{\mathop{\rm diag}}}
\def\dist{\mathop{\rm dist}}
\def\ddiv{\mathop{\rm div}}
\def\dom{\mathop{{\rm dom}}}
\def\epi{\mathop{\text{\'epi}}}
\def\intt{\mathop{\rm int}}
\def\inv{\mathop{\rm inv}}
\def\lin{\mathop{\rm lin}}
\def\isom{\mathop{\rm Isom}}
\def\range{\mathop{\rm Im}}
\def\sign{\mathop{\rm sign}}
\def\supp{\mathop{\rm supp}}
\def\trace{\mathop{\rm trace}}
\def\val{\mathop{\rm val}}
\def\var{\mathop{\rm var}}

\def\Inf{\mathop{\rm Inf}}
\def\Ker{\mathop{\rm Ker}}
\def\Min{\mathop{\rm Min}}
\def\Max{\mathop{\rm Max}}

\def\dw{\mathop{\delta w}}

%%%%%%%%%%%%%%%% UNDERLINED AND OVERLINED LIMINF AND LIMSUP %%%
\def\liminfu{\mathop{\underline{\lim}}}
\def\limsupo{\mathop{\overline{\lim}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NUMBERS %%%%%%%%%%%%%%%%%%
\def\half{\mbox{$\frac{1}{2}$}}
\def\sixinv{\mbox{$\frac{1}{6}$}}
\def\1B{{\bf  1}}
\def\sbdeux#1#2{\mbox{\scriptsize$#1$}\atop\mbox{\scriptsize$#2$}}
\def\sbtrois#1#2#3{\mbox{\scriptsize$#1$}\atop\mbox{\scriptsize$#2$}\atop\mbox{\scriptsize$#3$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  NUMBER SPACES  %%%%
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\gA}{\mathsf{A}}
\newcommand{\gG}{\mathsf{G}}
\newcommand{\gN}{\mathsf{N}}
\newcommand{\gT}{\mathsf{T}}
\newcommand{\gV}{\mathsf{V}}
\newcommand{\gE}{\mathsf{E}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sA}{\mathcal{A}}

% \def\cR{I\hspace{-1mm}R}

\def\cC{\mathbb{C}}
\def\cN{\mathbb{N}}
\def\cP{\mathbb{P}}
\def\cQ{\mathbb{Q}}
\def\cR{\mathbb{R}}
\def\cZ{\mathbb{Z}}

\newcommand{\cE}{I\!\!E}
% \newcommand{\cR}{I\!\! R} \newcommand{\cN}{I\!\!N}
\newcommand{\cRbar}{\bar {I\!\! R}}
\newcommand{\rbar}{\overline{\mathbb{R}}}
\newcommand{\rbartosn}{\rbar^{_{\scriptstyle\sN}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  ENVIRONMENTS %%%%%%%%%%%%%%%%%%
\newcommand\be{\begin{equation}}
\newcommand\ee{\end{equation}}
\newcommand\ba{\begin{array}}
\newcommand\ea{\end{array}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}

\newenvironment{paoplist}{\vspace{-1ex}\begin{list}{-}
{\itemsep 0mm \leftmargin 2mm \labelwidth 0mm}}
{\end{list} \vspace{-1ex}}

\newenvironment{myenumerate}{
\renewcommand{\theenumi}{\roman{enumi}}
\renewcommand{\labelenumi}{(\theenumi)}
\begin{enumerate}}{\end{enumerate}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  SPACING %%%%%%%%%%%%%%%%%%
\newcommand{\noi}{\noindent}
\newcommand{\bs}{\bigskip}
\newcommand{\ms}{\medskip}
\newcommand{\msn}{{\bigskip \noindent}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  MISC %%%%%%%%%%%%%%%%%%
\newcommand{\refeq}[1]{(\ref{#1})}
%\newcommand{\eqref}[1]{(\ref{#1})}

\def\ATT{\marginpar{$\leftarrow$}}

\def\rar{\rightarrow}
\def\fmap{\rightarrow}

\def\ds{\displaystyle}
\def\disp{\displaystyle}

\def\La{\langle}
\def\la{\langle}
\def\ra{\rangle}
%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mypsfig}[3]
           {\begin{figure}[hbtp]
            \centerline{\input #1}
            \caption{\rm{#2}} \label{#3}
            \end{figure}}








%%% EOF

